Towards Ontology-Mediated Planning with OWL DL Ontologies (Extended Version)

While classical planning languages make the closed-domain and closed-world assumption, there have been various approaches to extend those with DL reasoning, which is then interpreted under the usual open-world semantics. Current approaches for planning with DL ontologies integrate the DL directly into the planning language, and practical approaches have been developed based on first-order rewritings or rewritings into datalog. We present here a new approach in which the planning specification and ontology are kept separate, and are linked together using an interface. This allows planning experts to work in a familiar formalism, while existing ontologies can be easily integrated and extended by ontology experts. Our approach for planning with those ontology-mediated planning problems is optimized for cases with comparatively small domains, and supports the whole OWL DL fragment. The idea is to rewrite the ontology-mediated planning problem into a classical planning problem to be processed by existing planning tools. Different to other approaches, our rewriting is data-dependent. A first experimental evaluation of our approach shows the potential and limitations of this approach.

==> PDDL_rewritings.tex <==
	\begin{framed}
	\begin{subfigure}[t]{0.3\textwidth}
		\begin{verbatim}
(:derived (inconsistent)
   (and
      (holds stackBot blockA)
      (holds stackBot blockB) 
      (holds stackBot blockC)
   )
)
		\end{verbatim}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.67\textwidth}
	\begin{verbatim}
(:derived (fullHands ?r)
   (or
      (inconsistent)
      (and (= ?r stackBot) (or
          (and (holds stackBot blockA) (holds stackBot blockB))
          (and (holds stackBot blockA) (holds stackBot blockC))
          (and (holds stackBot blockB) (holds stackBot blockC))
      ))
   )
)
	\end{verbatim}
	\end{subfigure}
	\end{framed}	

